MultiFuser: Multimodal Fusion Transformer for Enhanced Driver Action Recognition

Driver action recognition, aiming to accurately identify drivers' behaviours, is crucial for enhancing driver-vehicle interactions and ensuring driving safety. Unlike general action recognition, drivers' environments are often challenging, being gloomy and dark, and with the development of sensors, various cameras such as IR and depth cameras have emerged for analyzing drivers' behaviors. Therefore, in this paper, we propose a novel multimodal fusion transformer, named MultiFuser, which identifies cross-modal interrelations and interactions among multimodal car cabin videos and adaptively integrates different modalities for improved representations. Specifically, MultiFuser comprises layers of Bi-decomposed Modules to model spatiotemporal features, with a modality synthesizer for multimodal features integration. Each Bi-decomposed Module includes a Modal Expertise ViT block for extracting modality-specific features and a Patch-wise Adaptive Fusion block for efficient cross-modal fusion. Extensive experiments are conducted on Drive&Act dataset and the results demonstrate the efficacy of our proposed approach.

==> Sec/0_abstract.legacy.tex <==
Driver Action Recognition (DAR) is crucial for enhancing driving safety and smart cabin development.
Unlike general action recognition, DAR faces the challenge of capturing drivers’ subtle body movements under significant field-of-view obstructions and changing light conditions.
Recognizing this, utilizing multi-modal sensors in car cabins could be greatly beneficial.
However, existing research primarily focuses on single-modal methods or basic late fusion multi-modality techniques.
In this paper, we propose a new multi-modal fusion transformer for enhanced driver action recognition, MultiFuser, capable of fully utilizing multi-modal information for DAR.
Our Multi-stream Encoder effectively extracts the intra-modality features of each modality, while the Cross-modality Fusion Decoder efficiently fuses these features to generate inter-modality features.
Both intra-modality and inter-modality features together form a comprehensive global representation of multi-modal videos.
% Besides, the model is pretrained on the NTU-RGBD dataset to improve the comprehensive feature extraction in respective modalities.
Experimental results on the benchmark Drive\&Act Dataset demonstrate that three-modality MultiFuser outperforms the state-of-the-art single-modality CTA-NET by 5.45\% and the four-modality MDBU by 8.65\% in terms of balanced accuracy.

==> tab/table4.tex <==
\begin{table}[t]
\caption{The results of different fusion strategies (Accuracy in \%).}
\begin{center}
\begin{tabular}{c|c c}
\hline
Modality & Mean-1 & Top-1 \\ 
\hline
Early fusion & 49.88 & 67.30 \\
Late fusion & 61.58 & 78.63 \\
FFB in-chain & 62.28 & 78.32 \\
FFB off-chain & \textbf{70.67} & \textbf{82.39} \\
\hline
\end{tabular}
\label{fusion methods table}
\end{center}
\end{table}
